Unrolling Plug-and-Play Gradient Graph Laplacian Regularizer for Image Restoration

Generic deep learning (DL) networks for image restoration like denoising and interpolation lack mathematical interpretability, require voluminous training data to tune a large parameter set, and are fragile in the face of covariate shift. To address these shortcomings, we build interpretable networks by unrolling variants of a graph-based optimization algorithm of different complexities. Specifically, for a general linear image formation model, we first formulate a convex quadratic programming (QP) problem with a new $\ell_2$-norm graph smoothness prior called gradient graph Laplacian regularizer (GGLR) that promotes piecewise planar (PWP) signal reconstruction. To solve the posed unconstrained QP problem, instead of computing a linear system solution straightforwardly, we introduce a variable number of auxiliary variables and correspondingly design a family of ADMM algorithms. We then unroll them into variable-complexity feed-forward networks, amenable to parameter tuning via back-propagation. More complex unrolled networks require more labeled data to train more parameters, but have better overall performance. The unrolled networks have periodic insertions of a graph learning module, akin to a self-attention mechanism in a transformer architecture, to learn pairwise similarity structure inherent in data. Experimental results show that our unrolled networks perform competitively to generic DL networks in image restoration quality while using only a fraction of parameters, and demonstrate improved robustness to covariate shift.

==> image/curve/zhu_image.tex <==
\begin{figure*}[t]
\begin{center}
    

% \subfloat[Generalization ability]{\includegraphics[width=0.41\linewidth]{image/curve/z.pdf}}
% \label{fig:curve1}
% \hfill
{\includegraphics[width=0.47\linewidth]{image/curve/psnr_plot2.png}}
\label{fig:curve2}
\hfill
% \subfloat[Covariance Shift]{\includegraphics[width=0.32\linewidth]{image/curve/3.pdf}}
% \label{fig:curve3}
% \hfill

\end{center}
\vspace{-0.1in}
\caption{Robustness to noise covariance shift. All models were trained on noise level $\sigma=15$ and tested at different noise levels.}
% \vspace{-0.3cm}
\label{fig:cov_shift}
\end{figure*}


==> image/deblurry/deblurry_image.tex <==
% \begin{figure*}
%     \centering
%     \footnotesize
%     % \vspace{-0.3cm}
% 	\begin{tabular}{c@{}c@{}c@{}c@{}c}
% % \vspace{-0.4mm}
%         \includegraphics[width=2.0cm,height=2.00cm] 
%         {image/deblurry/blurry.jpg}  & 
% 		  \includegraphics[width=2.00cm,height=2.00cm] 
%         {image/deblurry/RGTV.jpg}  & 
% 		  \includegraphics[width=2.00cm,height=2.00cm] 
%         {image/deblurry/FDN.jpg} & 
%           \includegraphics[width=2.00cm,height=2.00cm]
%        {image/deblurry/ircnn.jpg}  & 
%           \includegraphics[width=2.00cm,height=2.00cm] 
%         {image/deblurry/ours.jpg} \\
% % \vspace{-0.4mm}
%         (a) Blurry image & (b) RGTV / 28.83dB & (c) FDN / 29.81dB & (d) IRCNN / 33.29dB & (e)  UPnPGGLR  / 33.72dB    
% 	\end{tabular}
	
	
% % \vspace{0.05cm}
% 	\caption{Visual results comparison of different deblurring methods on \textit{Leaves}. The blur kernel size is 19×1919\times19. The noise level is 2.55.}
%  \vspace{-0.3cm}
% 	\label{fig:deblur}
% \end{figure*}

\begin{figure*}[t]
\centerline{\includegraphics[width=0.99\textwidth]{image/deblurry/deblur2.jpg}}
\vspace{-0.3cm}
\caption{Visual results comparison of different deblurring methods on \textit{Leaves}. The blur kernel size is $19\times19$. The noise level is 2.55($1\%$).}
\label{fig:deblur}
 % \vspace{-0.15in}
\end{figure*}

==> image/false_gradient.tex <==
%\begin{figure}[t]
%\centerline{\includegraphics[width=0.85\textwidth]{image/false_gradient2.jpg}}
%\vspace{-0.3mm}
%\caption{Visual comparison using DeepGGLR with and without removal of false gradients. (a) Noisy patch, (b) DeepGGLR with false gradients, (c) DeepGGLR with removing false gradients, (d) Ground-truth.}
%\label{fig:false}
 % \vspace{-0.3cm}
%\end{figure}


 \begin{figure}[t]
     \centering
     \scriptsize
     % \vspace{-0.3cm}
 	\begin{tabular}{c@{}c@{}c@{}c}

          \includegraphics[width=3cm,height=3cm] 
         {image/false_gradient/guass.png} %\hspace{0.01mm} 
         &  		  \includegraphics[width=3cm,height=3cm] 
         {image/false_gradient/blury11.png} &
         \includegraphics[width=3cm,height=3cm] 
         {image/false_gradient/false_g22.png}  
         \hspace{0.01mm}&
         \includegraphics[width=3cm,height=3cm] 
         {image/false_gradient/ref.png} 
         \\ 
         (a) Noisy, 23.39dB & (b) DeepGGLR*, 30.76dB &(c) DeepGGLR, 31.14dB & (d) Ground-truth \\
 		  
         
         %  (c) DeepGGLR, 31.14dB  & (d) Ground-truth\\

 	\end{tabular}
	
 \vspace{0.05cm}
 	\caption{Visual comparison using DeepGGLR with and without removal of false gradients. (a) Noisy patch, (b) DeepGGLR with false gradients, (c) DeepGGLR with removing false gradients, (d) Ground-truth.}
  % \vspace{-0.3cm}
 	\label{fig:false}
 \end{figure}






% \begin{figure}[t]
%     \centering
%     \footnotesize
%     \vspace{-0.3cm}
% 	\begin{tabular}{c@{}c@{}c}

%          \includegraphics[width=2.70cm,height=2.54cm] 
%         {image/false_gradient/guass.png} \hspace{0.01mm} & 
% 		  \includegraphics[width=2.70cm,height=2.54cm] 
%         {image/false_gradient/blury11.png} \hspace{0.01mm} & 
% 		  \includegraphics[width=2.70cm,height=2.54cm] 
%         {image/false_gradient/false_g22.png} \hspace{0.01mm} \\ 
%          (a) Noisy / 23.39dB & (b) DeepGGLR* / 30.76dB & (c) DeepGGLR / 31.14dB  \\

% 	\end{tabular}
	
% % \vspace{0.05cm}
% 	\caption{To denoise image in (a), DeepGGLR without / with detecting and removing false gradients are shown in (b) and (c), respectively. (c) is visually clearer than (c) with a better reconstruction PSNR.}
%  \vspace{-0.3cm}
% 	\label{fig:false}
% \end{figure}


==> image/fig_piece.tex <==
\begin{figure}
\centerline{\includegraphics[width=0.8\textwidth]{image/false_gradient_1D.png}}
\vspace{-0.3mm}
\caption{(a) A 1D 3-piece linear signal—the signal is continuous at $p_1 = 1$ and non-continuous at $p_1 = 2$. (b) Over-smoothness caused by GGLR using a false gradient at $p_1 = 2$.}
\label{fig:image2}
\end{figure}

==> image/interpolation/interpolation.tex <==
\begin{figure*}[t]
% \vspace{-0.15in}
\centerline{\includegraphics[width=0.99\textwidth]{image/interpolation/interpolation2.jpg}}
\vspace{-0.10in}
\caption{Visual comparision for $80\%$ missing pixels. Interpolation by UPnPGGLR looks less blocky and more natural.}
\label{fig:interpolation}
 \vspace{-0.15in}
\end{figure*}

==> image/real_denoise.tex <==

\begin{figure*}[t]
% \vspace{-0.15in}
\centerline{\includegraphics[width=0.99\textwidth]{image/real_denoise/denoise.jpg}}
\vspace{-0.3cm}
\caption{Real image denoising results using different methods on the RENOIR dataset.}
\label{fig:comp}
 % \vspace{-0.05in}
\end{figure*}

% \begin{figure*}[t]
%     \centering
%     \footnotesize
%     % \vspace{-0.3cm}
% 	\begin{tabular}{c@{}c@{}c@{}c@{}c@{}c}
% % \vspace{-0.4mm}
%         \includegraphics[width=2.90cm,height=2.90cm] 
%         {image/real_denoise/6_r/gauss.png} \hspace{-0.04mm} & 
% 		  \includegraphics[width=2.90cm,height=2.90cm] 
%         {image/real_denoise/6_r/DnCNN_train.png} \hspace{-0.04mm} & 
% 		  \includegraphics[width=2.90cm,height=2.90cm] 
%         {image/real_denoise/6_r/glr.png} \hspace{-0.04mm} & 
%           \includegraphics[width=2.90cm,height=2.90cm]
%        {image/real_denoise/6_r/gtvo.png} \hspace{-0.04mm} & 
%           \includegraphics[width=2.90cm,height=2.90cm] 
%         {image/real_denoise/6_r/gglr.png} \hspace{-0.04mm} & 
%           \includegraphics[width=2.90cm,height=2.90cm] 
%         {image/real_denoise/6_r/ref.png} \hspace{-0.04mm} \\
% % \vspace{-0.4mm}
%         (a) Noisy / 21.89dB & (b) CDnCNN / 30.81dB & (c) DeepGLR / 31.74dB & (d) DeepGTV / 31.85dB & (e) DeepGGLR / 32.13dB & (f) Ground-truth    \\

%         \includegraphics[width=2.90cm,height=2.90cm] 
%         {image/real_denoise/10_r/gauss.png} \hspace{-0.04mm} & 
% 		  \includegraphics[width=2.90cm,height=2.90cm] 
%         {image/real_denoise/10_r/DnCNN_train.png} \hspace{-0.04mm} & 
% 		  \includegraphics[width=2.90cm,height=2.90cm] 
%         {image/real_denoise/10_r/glr.png} \hspace{-0.04mm} & 
%           \includegraphics[width=2.90cm,height=2.90cm]
%         {image/real_denoise/10_r/gtvo.png} \hspace{-0.04mm} & 
%           \includegraphics[width=2.90cm,height=2.90cm] 
%         {image/real_denoise/10_r/gglr_after.png} \hspace{-0.04mm} & 
%           \includegraphics[width=2.90cm,height=2.90cm] 
%         {image/real_denoise/10_r/ref.png} \hspace{-0.04mm} \\


%          (a) Noisy / 23.35dB & (b) CDnCNN / 29.92dB & (c) DeepGLR / 29.85dB & (d) DeepGTV / 29.61dB & (e) DeepGGLR / 30.11dB & (f) Ground-truth    
        


% 	\end{tabular}
	
% % \vspace{0.05cm}
% 	\caption{Real image noise removal for the DENOIR dataset with different approaches.}

%  % \vspace{-0.3cm}
% 	\label{fig:comp}
% \end{figure*}



==> table/cross_domain.tex <==
% \begin{table}[t]
%  \vspace{-0.3cm}
% \caption{Cross-domain generalization for real image denoising.}
% \vspace{-0.15in}
% \label{tab3}
% \begin{center}
% \setlength{\tabcolsep}{3pt}

%  % 开始居中对齐
% \resizebox{0.7\columnwidth}{!}{
% \begin{tabular}{|c|ccccc|}
% \hline
% \multirow{2}{*}{Metric} & \multicolumn{5}{c|}{Method}                                   \\ \cline{2-6} 
%                         & \multicolumn{1}{c|}{CDnCNN}& \multicolumn{1}{c|}{IRCNN} & \multicolumn{1}{c|}{DeepGLR} & \multicolumn{1}{c|}{DeepGTV} & UPnPGGLR \\ \hline
% PSNR                    & \multicolumn{1}{c|}{27.34} & \multicolumn{1}{c|}{25.26} & \multicolumn{1}{c|}{30.25}   & \multicolumn{1}{c|}{30.14}   & \textbf{30.38}    \\ \hline
% SSIM                    & \multicolumn{1}{c|}{0.6779} & \multicolumn{1}{c|}{0.600} & \multicolumn{1}{c|}{0.809}  & \multicolumn{1}{c|}{0.808}  & \textbf{0.814}   \\ \hline
% \end{tabular}
% }
%  % 开始居中对齐
% \vspace{-0.3in}
% \end{center}
% \end{table}


\begin{table}
\caption{Cross-domain generalization for real image denoising.}
\vspace{-0.15in}
\label{tab3}
\begin{center}
\setlength{\tabcolsep}{3pt}

 % 开始居中对齐
\resizebox{0.7\columnwidth}{!}{
\begin{tabular}{c|ccccc}
\hline
\multirow{2}{*}{Metric} & \multicolumn{5}{c}{Method}                    \\ \cline{2-6} 
                        & CDnCNN & IRCNN & DeepGLR & DeepGTV & UPnPGGLR \\ \hline
PSNR                    & 27.34  & 25.26 & 30.25   & 30.14   & \textbf{30.38}    \\
SSIM                    & 0.678 & 0.600 & 0.809   & 0.808   & \textbf{0.814}    \\ \hline
\end{tabular}
}
 % 开始居中对齐
\vspace{-0.3in}
\end{center}
\end{table}

==> table/gauss_denoise.tex <==




\begin{table}[t]
% \vspace{-0.3cm}
\caption{
Average PSNR(dB) results of different methods for noise levels $15$, $25$, and $50$ on CBSD68 \cite{roth2009fields} and real noise dataset
RENOIR \cite{renoir} and Nam-CC15 \cite{nam2016holistic}. Note that the proposed UPnPGGLR demonstrates strong generalization ability.}
\vspace{-0.25in}
\label{tab2}
\begin{center}    
\setlength{\tabcolsep}{3pt}
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{l|c|ccc|c|c}
\hline
\multirow{2}{*}{Method} & Paras(M) & \multicolumn{3}{c|}{CBSD68 \cite{roth2009fields}}                                                                                              & RENOIR \cite{renoir}      & Nam-CC15 \cite{nam2016holistic}   \\ \cline{2-7} 
                        & -        & \multicolumn{1}{c|}{$\sigma=15$} & \multicolumn{1}{c|}{$\sigma=25$} & $\sigma=50$ & -           & -           \\ \hline
CDnCNN \cite{DnCNN}                  & 0.56     & \multicolumn{1}{c|}{33.90/0.929}              & \multicolumn{1}{c|}{31.22/0.883}              & 27.95/0.790              & 26.79/0.638 & 33.86/0.864 \\
IRCNN \cite{zhang2017learning}                  & 4.75     & \multicolumn{1}{c|}{33.87/0.928}              & \multicolumn{1}{c|}{31.18/0.882}              & 27.86/0.789              & 25.77/0.651 & 35.68/0.932 \\
FFDNet \cite{FFDNet}                & 0.67     & \multicolumn{1}{c|}{33.85/0.929}              & \multicolumn{1}{c|}{31.22/0.883}              & 27.98/0.792              & 29.19/0.762 & 34.00/0.906 \\
DeepGLR \cite{deepglr}                & 0.93     & \multicolumn{1}{c|}{33.75/0.926}              & \multicolumn{1}{c|}{31.13/0.881}              & 27.86/0.791              & 30.25/0.809 & 35.85/0.935 \\
DeepGTV \cite{deepgtv} & \textbf{0.10}     & \multicolumn{1}{c|}{31.80/0.927}      &\multicolumn{1}{c|}{31.08/0.879}  &\multicolumn{1}{c|}{27.90/0.791}   & 30.14/0.808          & 35.98/0.932          \\


DRUNet \cite{zhang2021plug}                 & 32.64    & \multicolumn{1}{c|}{34.30/0.934}              & \multicolumn{1}{c|}{31.69/0.893}              & 28.51/0.810              & 29.81/0.784 & 35.52/0.927 \\
Restormer \cite{Zamir2021RestormerET}              & 26.11     & \multicolumn{1}{c|}{\textbf{34.39/0.935}}              & \multicolumn{1}{c|}{\textbf{31.78/0.894}}              & \textbf{28.59/0.813}              & 29.55/0.780 & 35.32/0.921 \\
UPnPGGLR                &  0.23     & \multicolumn{1}{c|}{34.12/0.932}              & \multicolumn{1}{c|}{31.38/0.889}              & 28.15/0.802              & \textbf{30.38/0.814} & \textbf{36.26/0.939} \\ \hline
\end{tabular}
}
\end{center}
\vspace{-0.30in}
\end{table}



==> table/real_denoise.tex <==
% \begin{table}[t]

% \caption{Denoising results by different methods on real images (RENOIR dataset).}
% \label{tab1}
% \vspace{-0.15in}
% \setlength{\tabcolsep}{3pt}
% \begin{center}

% \resizebox{0.8\columnwidth}{!}{
% \begin{tabular}{|c|cccccc|}
% \hline
% {\multirow{2}{*}{Metric}} & \multicolumn{6}{c|}{Method}                                                                                                        \\ \cline{2-7} 
% \multicolumn{1}{|r|}{}                        & \multicolumn{1}{c|}{CBM3D}  & \multicolumn{1}{c|}{CDnCNN} & \multicolumn{1}{c|}{IRCNN} & \multicolumn{1}{c|}{DeepGLR} & \multicolumn{1}{c|}{DeepGTV} & UPnPGGLR \\ \hline
% Paras(M)                                          & \multicolumn{1}{c|}{-}  & \multicolumn{1}{c|}{0.56}  & \multicolumn{1}{c|}{0.19}   & \multicolumn{1}{c|}{0.93}   & \multicolumn{1}{c|}{\textbf{0.10}} & 0.23  
% \\ \hline
% PSNR                                          & \multicolumn{1}{c|}{28.29}  & \multicolumn{1}{c|}{31.61}  & \multicolumn{1}{c|}{31.69}   & \multicolumn{1}{c|}{31.72}   & \multicolumn{1}{c|}{31.64} &\textbf{32.11}    \\ \hline
% SSIM                                          & \multicolumn{1}{c|}{0.740} & \multicolumn{1}{c|}{0.843} & \multicolumn{1}{c|}{0.845}  & \multicolumn{1}{c|}{0.849} &\multicolumn{1}{c|}{0.846}  & \textbf{0.856}   \\ \hline
% \end{tabular}
% }
    
% \end{center}
% \vspace{-0.3in}
% \end{table}




\begin{table}[t]

\caption{Denoising results by different methods on real images (RENOIR dataset).}
\label{tab1}
\vspace{-0.1in}
\setlength{\tabcolsep}{3pt}
\begin{center}

\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{c|cccccc}
\hline
\multirow{2}{*}{Metric} & \multicolumn{6}{c}{Method}                            \\ \cline{2-7} 
                        & CBM3D \cite{BM3D} & CDnCNN \cite{DnCNN} & IRCNN \cite{zhang2017learning}& DeepGLR \cite{deepglr} & DeepGTV \cite{deepgtv} & UPnPGGLR \\ \hline
PSNR                    & 28.29 & 31.61  & 31.69 & 31.72   & 31.64   & \textbf{32.15}    \\ 
SSIM                    & 0.740 & 0.843  & 0.845 & 0.849   & 0.846   & \textbf{0.857}    \\ 
Paras(M)                & -     & 0.56   & 4.75  & 0.93    & \textbf{0.10}    & 0.23     \\ \hline
\end{tabular}
}
    
\end{center}
\vspace{-0.2in}
\end{table}
